Automated test generation to evaluate tool-augmented LLMs as conversational AI agents

Tool-augmented LLMs are a promising approach to create AI agents that can have realistic conversations, follow procedures, and call appropriate functions. However, evaluating them is challenging due to the diversity of possible conversations, and existing datasets focus only on single interactions and function-calling. We present a test generation pipeline to evaluate LLMs as conversational AI agents. Our framework uses LLMs to generate diverse tests grounded on user-defined procedures. For that, we use intermediate graphs to limit the LLM test generator's tendency to hallucinate content that is not grounded on input procedures, and enforces high coverage of the possible conversations. Additionally, we put forward ALMITA, a manually curated dataset for evaluating AI agents in customer support, and use it to evaluate existing LLMs. Our results show that while tool-augmented LLMs perform well in single interactions, they often struggle to handle complete conversations. While our focus is on customer support, our method is general and capable of AI agents for different domains.

==> plots/clients_histogram.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar, % Style of the bar chart
    % The following symbolic coordinates should match the actual client names from your CSV
    % If you have too many clients or they are not fixed, you might want to consider removing or adjusting this line.
    symbolic x coords={Internet Provider, E-commerce Platform, Financial Institution, Entertainment Website}, %
    xtick=data, % Specify ticks at data points
    nodes near coords, % Places the counts near the respective bars
    nodes near coords align={vertical}, % Aligning the node text
    xlabel={Client types},
    ylabel={Counts},
    width=\columnwidth,,
    x tick label style={
        rotate=45,
        anchor=east,
        font=\small
    } % This rotates the x-axis labels to prevent overlap if many clients
]
\addplot table[x=client, y=count, col sep=comma] {data/client_hist.csv};
\end{axis}
\end{tikzpicture}



